IPS/Zeta Correspondence for the Domany-Kinzel model

Previous studies presented zeta functions by the Konno-Sato theorem or the Fourier analysis for one-particle models, including random walks, correlated random walks, quantum walks, and open quantum random walks. Furthermore, the zeta functions for the multi-particle model with probabilistic or quantum interactions, called the interacting particle system (IPS), were also investigated. In this paper, we focus on the zeta function for a class of IPS, including the Domany-Kinzel model, which is a typical model of the probabilistic IPS in the field of statistical mechanics and mathematical biology.

==> backup.tex <==
In this proof, we only consider the case $N=3$, for the sake of the simplicity. However, similar discussion can be done for general $N\geq2$. First, we introduce $ 2\times 2$ matrices as follows:
\begin{align*}
E_{00} =\begin{bmatrix}
1 & \cdot \\
\cdot  & \cdot 
\end{bmatrix} ,\ \ E_{11} =\begin{bmatrix}
\cdot  & \cdot \\
\cdot  & 1
\end{bmatrix} , & \ \ E_{01} =\begin{bmatrix}
\cdot  & 1\\
\cdot  & \cdot 
\end{bmatrix} ,\ \ \ E_{10} =\begin{bmatrix}
\cdot  & \cdot \\
1 & \cdot 
\end{bmatrix} .
\end{align*}Additionally, we can see the following relationship from the definition.
\begin{align*}
Q^{( l)} & =\sum _{i_{1} ,i_{2} ,i_{3} ,i_{4}} a_{i_{3} i_{4}}^{i_{1} i_{2}} E_{i_{3} i_{1}} \otimes E_{i_{4} i_{2}} =\sum _{i,j,k} a_{jk}^{ik} E_{ji} \otimes E_{kk}.
\end{align*}
Then, we have
\begin{align*}
&Q_{3}^{( g)}  
\\
&=\left( I_{2} \otimes Q^{( l)}\right)\left( Q^{( l)} \otimes I_{2}\right)\\
 & =\left(I_{2} \otimes \left(\sum _{i_{2} ,j_{2} ,k_{2}} a_{j_{2} k_{2}}^{i_{2} k_{2}} E_{j_{2} i_{2}} \otimes E_{k_{2} k_{2}}\right)\right)\left(\left(\sum _{i_{1} ,j_{1} ,k_{1}} a_{j_{1} k_{1}}^{i_{1} k_{1}} E_{j_{1} i_{1}} \otimes E_{k_{1} k_{1}}\right) \otimes I_{2}\right)\\
 & =\sum _{i_{1} ,j_{1} ,k_{1}}\sum _{i_{2} ,j_{2} ,k_{2}} a_{j_{1} k_{1}}^{i_{1} k_{1}} a_{j_{2} k_{2}}^{i_{2} k_{2}}( I_{2} \otimes E_{j_{2} i_{2}} \otimes E_{k_{2} k_{2}})( E_{j_{1} i_{1}} \otimes E_{k_{1} k_{1}} \otimes I_{2})\\
 & =\sum _{i_{1} ,j_{1} ,k_{1}}\sum _{i_{2} ,j_{2} ,k_{2}} a_{j_{1} k_{1}}^{i_{1} k_{1}} a_{j_{2} k_{2}}^{i_{2} k_{2}}( E_{j_{1} i_{1}} \otimes E_{j_{2} i_{2}} E_{k_{1} k_{1}} \otimes E_{k_{2} k_{2}}) ,
\end{align*}
where if $ i_{2} \neq k_{1}$, $ E_{j_{2} i_{2}} E_{k_{1} k_{1}}$ is 
\begin{align*}
E_{j_{2} i_{2}} E_{k_{1} k_{1}} & =O_{2} .
\end{align*}
Furthermore, noting that $E_{j_{2} i_{2}} E_{i_{2} i_{2}} =E_{j_{2} i_{2}}$, then we take the trace of both sides, and we get 
\begin{align*}
\mathrm{tr}\left( Q_{3}^{( g)}\right) & =\sum _{i_{1} ,k_{1}}\sum _{i_{2} ,j_{2} ,k_{2}} a_{i_{1} k_{1}}^{i_{1} k_{1}} a_{j_{2} k_{2}}^{i_{2} k_{2}}\mathrm{tr}( E_{i_{1} i_{1}})\mathrm{tr}( E_{j_{2} i_{2}} E_{i_{2} i_{2}})\mathrm{tr}( E_{k_{2} k_{2}})\\
 & =\sum _{i_{1}}\sum _{i_{2} ,k_{2}} a_{i_{1} i_{2}}^{i_{1} i_{2}} a_{i_{2} k_{2}}^{i_{2} k_{2}}\mathrm{tr}( E_{i_{1} i_{1}})\mathrm{tr}( E_{i_{2} i_{2}})\mathrm{tr}( E_{k_{2} k_{2}})\\
 & =\sum _{i_{1}}\sum _{i_{2}}\sum _{i_{3}} a_{i_{1} i_{2}}^{i_{1} i_{2}} a_{i_{2} i_{3}}^{i_{2} i_{3}} .\ \ \end{align*}
